On the categorization of scientific citation profiles in computer sciences

A common consensus in the literature is that the citation profile of published articles in general follows a universal pattern - an initial growth in the number of citations within the first two to three years after publication followed by a steady peak of one to two years and then a final decline over the rest of the lifetime of the article. This observation has long been the underlying heuristic in determining major bibliometric factors such as the quality of a publication, the growth of scientific communities, impact factor of publication venues etc. In this paper, we gather and analyze a massive dataset of scientific papers from the computer science domain and notice that the citation count of the articles over the years follows a remarkably diverse set of patterns - a profile with an initial peak (PeakInit), with distinct multiple peaks (PeakMul), with a peak late in time (PeakLate), that is monotonically decreasing (MonDec), that is monotonically increasing (MonIncr) and that can not be categorized into any of the above (Oth). We conduct a thorough experiment to investigate several important characteristics of these categories such as how individual categories attract citations, how the categorization is influenced by the year and the venue of publication of papers, how each category is affected by self-citations, the stability of the categories over time, and how much each of these categories contribute to the core of the network. Further, we show that the traditional preferential attachment models fail to explain these citation profiles. Therefore, we propose a novel dynamic growth model that takes both the preferential attachment and the aging factor into account in order to replicate the real-world behavior of various citation profiles. We believe that this paper opens the scope for a serious re-investigation of the existing bibliometric indices for scientific research.

==> method.tex <==

\section{Materials and Methods}


% \subsection{Algorithm for Categorizing Citation Profiles}
% In order to identify the different categories of citation profile, we perform various processing on our dataset. First
% of all, to smoothen the time
% series data points in the citation profile of a paper, we use five-years moving average filtering; then, we scale the data points by
% normalizing them with the maximum value present in the time series (i.e, maximum citation received by the paper in some particular year);
% finally, we run local peak detection algorithm\footnote{{\tiny The peak detection algorithm is available
% in Matlab Spectral Analysis package - \url{http://www.mathworks.in/help/signal/ref/findpeaks.html}; we use `MINPEAKDISTANCE'=2 and
% `MINPEAKHEIGHT'=0.75 and the default values for the other parameters.}} to detect peaks in the citation profile. In addition, we apply
% the following two heuristics to specify peaks: (i) the height of a peak should be at least 75\% of the maximum peak-height, and (ii) two
% consecutive peaks should be separated by more than 2 years; otherwise they are treated as a single peak. 

% 
% \subsection{Core-periphery Analysis}
% We intend to measure the impact of those papers whose category information is known to us in the year 2000 (denoted by set $S$). Once the
% citations keep coming after 2000, the impact of papers in each category might also change which triggers the changes in the core periphery
% structure of the citation network. Therefore, we construct different cumulative citation networks in different years -- 2000, 2004, 2007
% and 2010
% such that citation network constructed in the year $Y$ contains the induced subgraph of all papers published at or before $Y$. Then for each
% such network, we run the following methods: 
% we start by recursively removing nodes that have a single inward link until no such nodes remain in the network. These nodes form the
% $1$-shell of the network ($k^s$-shell index $k^s = 1$). Similarly, by recursively removing all nodes with degree 2, we get the $2$-shell. We
% continue increasing $k$ until all nodes in the network have been assigned to one of the shells. The union of all the shells with index
% greater than or equal to $k^s$ is called the $k^s$-core of the network, and the union of all shells with index smaller or equal to $k^s$ is
% the $k^s$-crust of the network. 

\subsection{Dynamic Growth Model}
As mentioned earlier, unlike the standard growth models proposed previously for citation networks, our model takes into account
preferential attachment
\cite{Albert2002, Barabasi99, Price} and aging \cite{RePEc:eee} of each paper (denoted by the number of years since publication) in order to
synthesize the network. To begin with, we include the first six years (1970 - 1975 (inclusive)) network information from the real
dataset to bootstrap the model. This information includes -- induced
subgraph of the papers published within these years, their category
information and the year of publication. Apart from this, for fair comparison with the real-world dataset, we use two more distributions
generated from the real-world dataset -- year-wise distribution of the number of publications (denoted as {\em Pub-dist}) and the reference
distribution (i.e., number of references vs. fraction of papers having those many references, denoted as {\em Ref-dist}). These form the base
statistics of our model.

Since we know the category information of the papers which are considered in the base statistics, we form six buckets corresponding to the six categories. Each bucket
constitutes papers of the corresponding category. Now for inserting new papers in the network at each time step $t$ (corresponds to a
particular
year), we execute the following steps in order:\\
1. Select the actual number of papers (say, $N$) published at time $t$ from {\em Pub-dist}, and create a set of $N$ number of nodes (say,
$P_N$)
    to be inserted in the network.\\
2. For each such $p$ present in $P_N$:

\hspace{2 mm}  2.1 Select one of the buckets (categories) for $p$ preferen-

\hspace{8 mm}tially based on the size of the buckets.

\hspace{2 mm}  2.2 Select a value $R$ from {\em Ref-dist} to determine the num

\hspace{8 mm}ber 
of outward edges (references) emanating from $p$.

\hspace{2 mm}  2.3 For each outward edge, select the other end-point 

\hspace{8 mm}using the following steps:

\hspace{7 mm}  2.3.1  Select a bucket $B$ preferentially based on the 

\hspace{16 mm}number of incoming citations obtained by the 

\hspace{16  mm}papers in different
buckets till time $t-1$.

\hspace{7 mm}  2.3.2  Select one of the papers from $B$ based on its 

\hspace{16 mm} {\em attractiveness} at time $t-1$.

\hspace{2 mm}  2.4 Finally, assign $p$ in the selected category.



\noindent The {\em attractiveness ($\pi_i$)} of a paper $p_i$ is determined by the category where it falls using the two factors -- the time
after
its publication (aging) and the total citation count it has accumulated so far (preferential attachment) as follows. The notations used to
describe the formulation of $\pi_i$ for the different categories are -- $k_i$: the in-degree of paper $p_i$, $\mu$: average citation count of papers present in the
category where $p_i$ belongs to,
$\rho$: a parameter of the 
model used to dampen certain factors associated with it, $\tau$: a
%PG: \rho definition not clear
parameter of the model used to scale the time of occurrences of the peaks.


\begin{itemize}
 \item \textbf{MonDec:} Each paper declines in its popularity exponentially with time but remains proportional to its overall
significance, i.e., \\
\begin{center}
 $ \pi_{i} = \frac{k_{i} + \mu} { \exp ({\rho t}) }; \ \forall t $
\end{center}






\item \textbf{PeakInit:} We assume $T$ as the occurrence of the early peak in such distribution. PeakInit pattern comprises two phases as
commonly hypothesized for most of the earlier papers -- initial increase through preferential attachment and then a continuous decline.
Therefore,
\begin{center}
 $\pi_{i} = k_{i} + \mu;\ if\ t \leq T + \tau$\\
$\pi_{i} = \frac{k_{i} + \mu} { \rho t } ; \ otherwise $
\end{center}

\item {\bf LatePeak:}  We assume $T$ as the occurrence of the late peak in such distribution. PeakLate behaves similarly as PeakInit with
the only difference that it experiences its peak at a much later period after the time of publication. Therefore,
\begin{center}
$\pi_{i} = k_{i} + \mu;\  if\ t \leq T+\tau$\\
$\pi_{i} = \frac{k_{i} + \mu} { \rho t } ;\ otherwise $
\end{center}


\item \textbf{PeakMul:} We observe that about 65.04\% papers in PeakMul category have two peaks on an average in the timeline of the
citation profile (see SI text). Therefore, in this model we assume that $T_1$ and $T_2$ are
the times of two peaks respectively. The pattern of this profile can be
sub-divided into four phases -- initial rise through preferential attachment followed by a
monotonic decline, a second rise through preferential attachment followed by a monotonic decline. Therefore, 
\begin{center}
$\pi_{i} = k_{i} + \mu ; \  if\ 0 \leq t \leq T_1+\tau$\\
$\pi_{i} = \frac{k_{i} + \mu} { t } ;\  if \ T_1+\tau < t \leq \frac{T_1+T_2}{2}+\tau$\\
$\pi_{i} = k_{i} + \mu ;\ if \ \frac{T_1+T_2}{2}+\tau < t \leq T_2+\tau$\\
$\pi_{i} = \frac{k_{i} + \mu} { t };\ otherwise $
\end{center}





\item \textbf{MonIncr:} In this category, each paper acquires popularity directly proportional to its earlier citation count as well as
time. Thus,
\begin{center} 
$\pi_{i} = k_{i} + \rho \mu + t   ;\  \forall t $\\
\end{center}

\item \textbf{Oth:} Since the papers in this category do not follow any particular pattern of citation profile, we do not add the aging
factor here. When a new added paper tries to connect the references to the papers in this category, the papers are selected uniformly at
random, i.e., the $\pi$ values for all the papers in this category are same and remain constant over time.  


\end{itemize}
The values of $\pi$ for each paper and $\mu$ for each category are calculated on the fly at each time $t$ based on the information at time
$t-1$. The time of occurrences of peaks ($T$, $T_1$ and $T_2$) are selected from the actual distribution of peak occurrence
time for each category individually. The results in Figure \ref{profile} (bottom panel) are reported after
averaging the results over 100 simulations. The final values of the
model parameters determined in order to closely match the simulation results with the real-world patterns are as follows: $\tau$ = 1
(PeakInit) and =3 (rest); $\rho$ = 0.25 (MonDec), =0.7 (PeakInit), =0.5 (PeakLate) and =0.3 (MonIncr). 








 
